FlowDreamer: Exploring High Fidelity Text-to-3D Generation via Rectified Flow

Recent advances in text-to-3D generation have made significant progress. In particular, with the pretrained diffusion models, existing methods predominantly use Score Distillation Sampling (SDS) to train 3D models such as Neural RaRecent advances in text-to-3D generation have made significant progress. In particular, with the pretrained diffusion models, existing methods predominantly use Score Distillation Sampling (SDS) to train 3D models such as Neural Radiance Fields (NeRF) and 3D Gaussian Splatting (3D GS). However, a hurdle is that they often encounter difficulties with over-smoothing textures and over-saturating colors. The rectified flow model -- which utilizes a simple ordinary differential equation (ODE) to represent a straight trajectory -- shows promise as an alternative prior to text-to-3D generation. It learns a time-independent vector field, thereby reducing the ambiguity in 3D model update gradients that are calculated using time-dependent scores in the SDS framework. In light of this, we first develop a mathematical analysis to seamlessly integrate SDS with rectified flow model, paving the way for our initial framework known as Vector Field Distillation Sampling (VFDS). However, empirical findings indicate that VFDS still results in over-smoothing outcomes. Therefore, we analyze the grounding reasons for such a failure from the perspective of ODE trajectories. On top, we propose a novel framework, named FlowDreamer, which yields high fidelity results with richer textual details and faster convergence. The key insight is to leverage the coupling and reversible properties of the rectified flow model to search for the corresponding noise, rather than using randomly sampled noise as in VFDS. Accordingly, we introduce a novel Unique Couple Matching (UCM) loss, which guides the 3D model to optimize along the same trajectory.

==> intro_old_version_backup.tex <==
3D assets are already ubiquitous in our lives, helping us to visualize complex scenes or objects more easily. 
% Recently, the techniques of text-to-3D have developed rapidly.
% The 3D assets by created by text-to-3D are also embedded in game and movie production, lowering the barrier for non-professionals and providing more opportunities for amateur 3D modelers to create 3D assets.
% % （先说一下3D assert的好处）
% Although text-to-3D can be applied in many areas, it still has a lot of challenges to be solved. 
% It requires a lot of time, effort, and resources to optimize 3D objects and generated 3D assets is over-smooth and lack details.
% % （转折一下，说一下3D 的困难）
% The availability of open-source 3D data is much less than that of text and image paired datasets, which has also somewhat hindered the development of text-to-3D.
% % 先说一下这个text-to-image的发展，然后说到text-to-3D为什么发展没有那么快。
% With the rapid development of text-to-image \cite{ddpm,songddim,song2020score,clip,saharia2022imagen}, which has achieved great success.
% Dreamfusion \cite{dreamfusion} propose a novel Score Distillation Sampling(SDS) loss utilizing a pretrained text-to-image diffusion model\cite{ddpm,songddim} as guidance to optimize 3D model NeRF\cite{nerf}.
% % SDS use noise residual 
% % SDS leverages the ability of diffusion models to gradually optimize a low-quality image into a high-quality one to update parameterized 3D renders. 
% %（这句话只是很大致描述，大概率有问题）
% % we instead want to create 3D models that look like good images when rendered from random angles.(这里这句话是来自dreamfusion原文，后面需要加入)

% % 然后提一下flow generative model 的发展，
% With the rapid development of flow generative models\cite{dinh2014niceflow,kingma2018glow,liu2022rcflow,lipman2022flowmatching,liu2023instaflow}, the study of text-to-3D with flow generative model as guidance is very necessary.
% %(这里第一个研究可能描述不对)
% We imitate Dreamfusion\cite{dreamfusion} to use SDS loss with flow generative model as guidance to optimize 3D model\cite{nerf,3dgs}, we called it Rc-SDS.
% % we almost the pioneer in researching that it is still possible to use SDS to optimize 3D rendering under the flow generative model.

% We find Rc-SDS still has some issues like over-smoothing, lack details and slow convergence.%(说了SDS在flow中任然有问题)
% In this paper, we thoroughly investigate the underlying cause of these issues when using Rectified flow generative models as guidance. %（再说一下，造成这些问题的原因在flow下）
% % 下面就是证明描述就有很大问题。到底要不要避开数学公式，所以我先refine our approach


% % (然后在这里放入SDS表达式， (x0-x1)- v(xt,t), x0~N(0,1), x1=g(@),这里到底要不要直接放入公式呢，还是文字描述呢。)

% % 我们发现在flow-based generative model 直接采用SDS，会引入额外的噪声,从而导致收敛十分缓慢，以及过于平滑以及细节缺失等问题。
% % \ref{} shows that SDS distillation process by sampling $x_0$ and $t$, and interpolate $x_t$ using $x_0$ and $g(\theta, c)$, such that $x_t$ is obtained as $x_t = t \cdot x_0 + (1-t) \cdot g(\theta, c)$, which is then fed into the $v(x_t,t)$ to obtain the gradient at $x_t$ for updating $g(\theta,c)$.
% Rc-SDS distillation process involves sampling $x_0$ and $t$ and every optimization needs to sample $x_0$.
% While a trained Rectified generative model has the characteristic of causality\cite{liu2022rcflow}, which represents $x_0$ sample from Gaussian distribution $pi_0$ and $x_0$ sample from data distribution $\pi_1$ form a couple, $couple(x_0,x_1)$.
% Every couple is unique, which means that the trajectory from $x_0$ to $x_1$ is 
% determined in the same trained Rectified flow generative model.
% The $x = g(\mathbf{\theta, c})$ is determined in every optimization in Rectified flow model but Rc-SDS sample a new $x_0$ from $\mathcal{N}(\mathbf{0}, \mathbf{I})$.
% So every optimization forms a new $couple(x_0,x)$, which represents every optimization is on different trajectories.
% Optimizing the different trajectories leads to optimizing the average of these different trajectories\ref{fig:trajectory}, which causes over-smooth, slow convergence and lack details.

% % In this paper, to overcome the issues of the aforementioned. we propose a novel approach called Couple Matching (CP).
% % (CP) 利用了flow 双射性质 to get its couple x0, which makes the trajectory 一致. which 避免了不同轨迹下梯度的方向差异带来的slow convergence and oversmooth. And 为了 to get couple $x_0$, we design some expirents to find that we can just use few steps in logn time schedule, which 就能得到很好的效果。
% In this paper, to overcome the issues mentioned above, we propose a novel loss called \textit{\textbf{Couple loss}}. 
% \textit{\textbf{Couple loss}} utilizes the characteristics of reversibility and causality to make the trajectory consistent in every optimization.
% Rectified flow is an ordinary differential equation (ODE)\cite{chen2018ode} solver,$v_\phi(x_t,t)$. We can use the reversibility and causality of Rectifiel flow model to reverse the gradient of the $v_\phi(x_t,t)$ to find a $x'_0$ to form a new $couple(x'_0,x)$.
% Because the causality of Rectified flow model, if $x$ is determined then $x'_0$ is determined. 
% $couple(x'_0,x)$ make the trajectory consistent in every optimization, which avoids over-smooth, slow convergence and lack details.
% To obtain the $couple(x'_0,x)$, we design some experiments and find that using only 3 steps in Euler method can yield very good results.

% % bijective nature of flow models to obtain its counterpart $x_0$, which makes the trajectory consistent. %(里面的双射， 我后面会好好看)
% % This avoids the issues of slow convergence and over-smoothing caused by gradient direction differences across different trajectories. 
% % To obtain the couple $x_0$, we designed some experiments and found that using only a few steps in a logarithmic time schedule can yield very good results. %(这里后面可能要写出来steps)

% % Our expirents use point-e\cite{} to initilizate gaussian splatting for better 质量 和 save training time. We also use nerf for our 3D model, but find that it can't get a stable results. For this 现象，we deeply 分析了 the reason, we use a warm up phasa to make it more stable. Our method achieves a new state-of-the-art performance in text-to-3D tasks both in nerf and gaussian splatting.
% Our experiments use Point-E \cite{nichol2022point_e} to initialize Gaussian splatting for better quality and to save training time. 
% It can achieve high-quality results directly using \textit{\textbf{couple loss}}.
% We also use NeRF for our 3D model but find that it can't achieve stable results. 
% For this phenomenon, we deeply analyze the reason and implemented a warm-up phase to make it more stable. 
% Our method achieves a new state-of-the-art performance in text-to-3D tasks in both NeRF and Gaussian splatting\cite{chen2023gaussiansplatting}.
% % 我们发现在Nerf和gaussian splatting上有不同的结果。gaussian splatting 采用 point-e直接初始化可以运用我们的couple loss，而在nerf中直接采用couple loss会导致失败，我们深入分析了nerf直接采用couple loss失败的原因，并且采用了一个warm up的过程，使其在nerf generation 中更加稳定。经过对比，our method achieves a new state-of-the-art performance in text-to-3D tasks.
% % Overall, our contributions can be summarized as follows.
% % 1。Recently，我们是第一个在flow-based generative model 下，深入分析Score Distillation Sampling (SDS) 在 text-to-3D tasks中产生收敛过慢，以及过于平滑等问题的原因。
% % 2。对于SDS产生的问题，我们推出了couple matching loss，使其每次更新都在同一条轨迹上，使其梯度方向一致，从而加快了收敛速度以及提高了生成的质量。
% % 3。我们在nerf，gaussian splatting 下均采取了couple matching实验，并且深入分析了nerf 与 gaussian splatting不同的初始化造成的差异，然后分析差异，并且对nerf采用了warn up 使其generation 更加稳定。
% Overall, our contributions can be summarized as follows:
% \begin{itemize}
% \item We are the first to deeply analyze the reasons for slow convergence and over-smoothing issues of Score Distillation Sampling (SDS) in text-to-3D tasks under flow-based generative models.
% \item To overcome the issues of SDS, we propose a novel \textit{\textbf{couple loss}}, ensuring the trajectory consistent in each optimization, which aligns the gradient directions, thereby accelerating convergence and improving generated quality.
% \item We conducted \textit{\textbf{couple loss}} under both NeRF and 3D Gaussian splatting, deeply analyzing the differences between NeRF and Gaussian splatting. Based on this analysis, we implemented a warm-up phase for NeRF to make its generation more stable.
% \end{itemize}

